Parallelizing Workload Execution in Embedded and High-Performance Heterogeneous Systems

In this paper, we introduce a software-defined framework that enables the parallel utilization of all the programmable processing resources available in heterogeneous system-on-chip (SoC) including FPGA-based hardware accelerators and programmable CPUs. Two platforms with different architectures are considered, and a single C/C++ source code is used in both of them for the CPU and FPGA resources. Instead of simply using the hardware accelerator to offload a task from the CPU, we propose a scheduler that dynamically distributes the tasks among all the resources to fully exploit all computing devices while minimizing load unbalance. The multi-architecture study compares an ARMV7 and ARMV8 implementation with different number and type of CPU cores and also different FPGA micro-architecture and size. We measure that both platforms benefit from having the CPU cores assist FPGA execution at the same level of energy requirements.

==> benchmarks.tex <==
\section{Benchmarks}\label{sec:BENCH}
The benchmarks are written in C/C++ for both CPU and FPGA targets and the FPGA benchmarks are compiled using the high-level synthesis tools part of the SDSoC framework. Unfortunately, although the code is functionally portable it is not generally performance portable and the source code needs to be re-factor to suit the architecture of the FPGA device.


==> platform.tex <==
\section{Simultaneous multiprocessing SDSoC platform. Hardware Description}
\label{sec:PLAT}

%\subsection{Hardware description}

The SDSoC environment is able to generate hardware acceleration blocks that run on the FPGA, that can integrate DMA engines to autonomously read input data and write output data without a host thread intervention. The host thread and the accelerator manage the communication status using memory mapped registers, which are accessed through a slave interface of the AXI\_LITE communication bus. Additional master interfaces are typically implemented in the acceleration block to read the input and output data from and to main memory as it is processed.

% Dario, Removed this sentence because it seems the host is pooling the register 
%The host monitors the contents of these registers to determine when the IP block has completed its operation. 

%In the proposed platform, a dedicated AXI memory-mapped interface enables the acceleration hardware block to generate software defined interrupts to the host thread once processing has completed on the FPGA. This removes the need for the host to constantly pool the status of the hardware registers for completion using the default slave interface and effectively frees one CPU core for other tasks. 

SDSoC offers \texttt{async} and \texttt{wait} pragmas to enable asynchronous execution on the FPGA so that the hardware function returns control immediately to the host thread. Once the host thread reaches the \texttt{wait} pragma it enters into a spin-lock and it is continuously busy waiting for the hardware (FPGA) to complete. This is inefficient since the CPU core that allocates the host thread cannot perform any useful work and consumes energy with 100\% utilization. %Removed by MA: it does not add to the discussion
%To perform useful work until the \texttt{wait} statement is reached requires to exactly measure hardware execution time and allocate the correct amount of work to the host thread, otherwise load unbalancing inefficiencies will take place. 

To address that problem, this work proposes extending the SDSoC framework with an interrupt mechanism. To do that, a dedicated AXI memory-mapped interface enables the acceleration hardware block to generate interrupts to the host thread once processing has completed on the FPGA. This removes the need for the host thread to constantly poll the status of the hardware registers for completion using the default slave interface and effectively frees one CPU core for other tasks. That is, after asynchronously launching the hardware function, the host thread will yield voluntarily the CPU by changing to the sleeping state. After that, it will only wake up once the hardware accelerator has completed its task. During this sleep time, the dynamic scheduler proposed in Section~\ref{sec:progenv} is able to allocate another working thread to the running state to perform useful work in the CPU core left idle (see Fig.\ref{fig:platform}(b)). To enable this approach, a new hardware platform is proposed consisting of an additional IP block capable of generating shared interrupts to the main processor as illustrated in Fig.~\ref{fig:platform}(a).  

\begin{figure}[htb]
\centering
\begin{subfigure}[c]{.55\textwidth}
\includegraphics[width=\textwidth]{platform2.pdf}
  \subcaption{Hardware architecture}
  \label{fig:DB}
\end{subfigure}
\begin{subfigure}[c]{.43\textwidth}
\includegraphics[width=\textwidth]{cpu_fpga_flow.pdf}
\subcaption{Asynchronous offloading\protect\footnotemark}
\end{subfigure}
\caption{SDSoC multiprocessing platform. CC and FC stand for ``CPU core'' and ``FPGA Compute Unit'', respectively.}
\label{fig:platform}
\end{figure}
\footnotetext{For the sake of simplicity, the operating system activity has been excluded from the figure.}
The proposed IP is based on an AXI GPIO block whose interrupt line connects through a concatenate block (CONCAT) to the processor interrupt inputs. The Linux kernel driver created by SDSoC for the GPIO is replaced with a custom kernel driver capable of putting the host thread to sleep when asked to do so by the user application. Once the hardware block completes its operation, it writes an AXI GPIO register that generates the interrupt causing the host thread to wake up. 


\begin{figure}[hbt]
\centering
\begin{minipage}{0.92\linewidth}
\begin{lstlisting}[style=C]
//.h 
void mmult(float * in_a, float * in_b, float * out_c, int begin, int end, int *scalar,int *status, int enable);
//.cpp
 #pragma SDS async(1) (*@\label{list:async}@*)
  mmult(in_a, in_b, out_c, begin, end, scalar, status, enable); 
  ret_value = ioctl(file_desc, IOCTL_WAIT_INTERRUPT,0); (*@\label{list:ioctl}@*)
 #pragma SDS wait(1) (*@\label{list:wait}@*)
\end{lstlisting}
\end{minipage}
\caption{Prototype and invocation for hardware function \texttt{mmult}}
\label{fig:sleep}
\end{figure}

The code snippet of Fig.~\ref{fig:sleep} shows the function declaration and calling style for a hardware function called \texttt{mmult}. The first three parameters of \texttt{mmul} hardware function are pointers identifying the input/output memory areas which the function uses to receive/send data, while %\texttt{line\_count} 
\texttt{begin} and \texttt{end} will be used to define how much data in these memory areas must be processed. SDSoC constraints require that since the call to the hardware function uses the \texttt{async}/\texttt{wait} pragmas (lines~\ref{list:async} and~\ref{list:wait}), the function prototype cannot contain a return value. An additional value must be supplied in the function prototype, called \texttt{scalar} in this example, that will be modified by the hardware function. This \texttt{scalar} is implemented using AXI\_LITE interface and read by the host thread to learn when hardware processing has completed. The slave interface type AXI\_LITE means that this parameter cannot be used to generate the interrupt since it will only be read during the execution of \texttt{wait} pragma. The mechanism for interrupt generation itself needs a master interface that can write the GPIO register without the intervention of the host. To solve this problem an additional pointer is introduced in the function prototype called \texttt{status} that will be implemented as an AXIMM master interface. 
 \texttt{status} points to the AXI GPIO register that controls interrupt generation and is written by the IP once the processing has completed. Then the AXI GPIO can generate an interrupt to the host processor hence waking up the host thread. In the code we can also see the Linux \texttt{ioctl} function (line~\ref{list:ioctl}) that will ask the kernel driver to put the host thread to sleep until the arrival of the interrupt. Finally, the \texttt{enable} parameter is used to control if the IP block is able to generate interrupts. If this parameter is passed with value 1, the IP can generate interrupts otherwise interrupt generation is disabled.  % does not fit Notice that the original \texttt{wait} is still present. This acts as a safety mechanism with more than one hardware core and prevents execution from proceeding until all the cores in addition to the one that generated the interrupted have completed execution.

